Unsupervised Topic Segmentation of Meetings with BERT Embeddings

Topic segmentation of meetings is the task of dividing multi-person meeting transcripts into topic blocks. Supervised approaches to the problem have proven intractable due to the difficulties in collecting and accurately annotating large datasets. In this paper we show how previous unsupervised topic segmentation methods can be improved using pre-trained neural architectures. We introduce an unsupervised approach based on BERT embeddings that achieves a 15.5% reduction in error rate over existing unsupervised approaches applied to two popular datasets for meeting transcripts.

==> Makefile <==
.PHONY: FORCE all clean distclean

ifndef TARGET
TARGET=main
endif
.SUFFIXES: .pdf .ps .dvi .tex
.PHONY: clean distclean 

all: $(TARGET).pdf

%.pdf: %.tex FORCE
	latexmk -pdf -pdflatex="pdflatex -synctex=1" -use-make $(TARGET).tex

clean:
	for ext in aux log toc lof lot lol dlog bbl blg out tpt fdb_latexmk; \
	do \
		$(RM) $(TARGET).$$ext ; \
	done
	$(RM) *.aux *.bak *~

distclean: clean
	$(RM) $(TARGET).pdf
	$(RM) *.d

